Model-Driven Rapid Prototyping for Control Algorithms with the GIPS Framework (System Description)

Software engineers are faced with the challenge of creating control algorithms for increasingly complex dynamic systems, such as the management of communication network topologies. To support rapid prototyping for these increasingly complex software systems, we have created the GIPS (Graph-Based ILP Problem Specification) framework to derive some or even all of the building blocks of said systems, by using Model-Driven Software Engineering (MDSE) approaches. Developers can use our high-level specification language GIPSL (Graph-Based ILP Problem Specification Language) to specify their desired model optimization as sets of constraints and objectives. GIPS is able to derive executable (Java) software artifacts automatically that optimize a given input graph instance at runtime, according to the specification. Said artifacts can then be used as system blocks of, e.g., topology control systems. In this paper, we present the maintenance of (centralized) tree-based peer-to-peer data distribution topologies as a possible application scenario for GIPS in the topology control domain. The presented example is implemented using open-source software and its source code as well as an executable demonstrator in the form of a virtual machine is available on GitHub.

==> eptcsdata.tex <==
\providecommand{\firstpage}{157}
\providecommand{\publicationstatus}{J. Endrullis, D. Grzelak, T. Heindel and J. Kosiol (Eds):\\ GCM 2023 and GCM 2024\\
EPTCS 417, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.417.9}{10.4204/EPTCS.417.9}}
\pdfoutput=1

